Search for the Rare Decay B->K nu nubar

We present a search for the rare decays B+ -> K+ nu nubar and B0 -> K0 nu nubar using 459 million BBbar pairs collected with the BaBar detector at the SLAC National Accelerator Laboratory. Flavor-changing neutral-current decays such as these are forbidden at tree level but can occur through one-loop diagrams in the Standard Model (SM), with possible contributions from new physics at the same order. The presence of two neutrinos in the final state makes identification of signal events challenging, so reconstruction in the semileptonic decay channels B -> D(*) l nu of the B meson recoiling from the signal B is used to suppress backgrounds. We set an upper limit at the 90% confidence level of 1.3 x 10^{-5} on the total branching fraction for B+ -> K+ nu nubar, and 5.6 x 10^{-5} for B0 -> K0 nu nubar. We additionally report partial branching fractions in two ranges of di-neutrino mass squared for B+ -> K+ nu nubar.

==> acknowledgements.tex <==
We are grateful for the 
extraordinary contributions of our \pep2\ colleagues in
achieving the excellent luminosity and machine conditions
that have made this work possible.
The success of this project also relies critically on the 
expertise and dedication of the computing organizations that 
support \babar.
The collaborating institutions wish to thank 
SLAC for its support and the kind hospitality extended to them. 
This work is supported by the
US Department of Energy
and National Science Foundation, the
Natural Sciences and Engineering Research Council (Canada),
the Commissariat \`a l'Energie Atomique and
Institut National de Physique Nucl\'eaire et de Physique des Particules
(France), the
Bundesministerium f\"ur Bildung und Forschung and
Deutsche Forschungsgemeinschaft
(Germany), the
Istituto Nazionale di Fisica Nucleare (Italy),
the Foundation for Fundamental Research on Matter (The Netherlands),
the Research Council of Norway, the
Ministry of Education and Science of the Russian Federation, 
Ministerio de Ciencia e Innovaci\'on (Spain), and the
Science and Technology Facilities Council (United Kingdom).
Individuals have received support from 
the Marie-Curie IEF program (European Union), the A. P. Sloan Foundation (USA) 
and the Binational Science Foundation (USA-Israel).



==> authors_may2010.tex <==
%% author list as of 03-May-2010 (442 authors)
%
\author{P.~del~Amo~Sanchez}
\author{J.~P.~Lees}
\author{V.~Poireau}
\author{E.~Prencipe}
\author{V.~Tisserand}
\affiliation{Laboratoire d'Annecy-le-Vieux de Physique des Particules (LAPP), Universit\'e de Savoie, CNRS/IN2P3,  F-74941 Annecy-Le-Vieux, France}
\author{J.~Garra~Tico}
\author{E.~Grauges}
\affiliation{Universitat de Barcelona, Facultat de Fisica, Departament ECM, E-08028 Barcelona, Spain }
\author{M.~Martinelli$^{ab}$}
\author{A.~Palano$^{ab}$ }
\author{M.~Pappagallo$^{ab}$ }
\affiliation{INFN Sezione di Bari$^{a}$; Dipartimento di Fisica, Universit\`a di Bari$^{b}$, I-70126 Bari, Italy }
\author{G.~Eigen}
\author{B.~Stugu}
\author{L.~Sun}
\affiliation{University of Bergen, Institute of Physics, N-5007 Bergen, Norway }
\author{M.~Battaglia}
\author{D.~N.~Brown}
\author{B.~Hooberman}
\author{L.~T.~Kerth}
\author{Yu.~G.~Kolomensky}
\author{G.~Lynch}
\author{I.~L.~Osipenkov}
\author{T.~Tanabe}
\affiliation{Lawrence Berkeley National Laboratory and University of California, Berkeley, California 94720, USA }
\author{C.~M.~Hawkes}
\author{A.~T.~Watson}
\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom }
\author{H.~Koch}
\author{T.~Schroeder}
\affiliation{Ruhr Universit\"at Bochum, Institut f\"ur Experimentalphysik 1, D-44780 Bochum, Germany }
\author{D.~J.~Asgeirsson}
\author{C.~Hearty}
\author{T.~S.~Mattison}
\author{J.~A.~McKenna}
\affiliation{University of British Columbia, Vancouver, British Columbia, Canada V6T 1Z1 }
\author{A.~Khan}
\author{A.~Randle-Conde}
\affiliation{Brunel University, Uxbridge, Middlesex UB8 3PH, United Kingdom }
\author{V.~E.~Blinov}
\author{A.~R.~Buzykaev}
\author{V.~P.~Druzhinin}
\author{V.~B.~Golubev}
\author{A.~P.~Onuchin}
\author{S.~I.~Serednyakov}
\author{Yu.~I.~Skovpen}
\author{E.~P.~Solodov}
\author{K.~Yu.~Todyshev}
\author{A.~N.~Yushkov}
\affiliation{Budker Institute of Nuclear Physics, Novosibirsk 630090, Russia }
\author{M.~Bondioli}
\author{S.~Curry}
\author{D.~Kirkby}
\author{A.~J.~Lankford}
\author{M.~Mandelkern}
\author{E.~C.~Martin}
\author{D.~P.~Stoker}
\affiliation{University of California at Irvine, Irvine, California 92697, USA }
\author{H.~Atmacan}
\author{J.~W.~Gary}
\author{F.~Liu}
\author{O.~Long}
\author{G.~M.~Vitug}
\affiliation{University of California at Riverside, Riverside, California 92521, USA }
\author{C.~Campagnari}
\author{T.~M.~Hong}
\author{D.~Kovalskyi}
\author{J.~D.~Richman}
\affiliation{University of California at Santa Barbara, Santa Barbara, California 93106, USA }
\author{A.~M.~Eisner}
\author{C.~A.~Heusch}
\author{J.~Kroseberg}
\author{W.~S.~Lockman}
\author{A.~J.~Martinez}
\author{T.~Schalk}
\author{B.~A.~Schumm}
\author{A.~Seiden}
\author{L.~O.~Winstrom}
\affiliation{University of California at Santa Cruz, Institute for Particle Physics, Santa Cruz, California 95064, USA }
\author{C.~H.~Cheng}
\author{D.~A.~Doll}
\author{B.~Echenard}
\author{D.~G.~Hitlin}
\author{P.~Ongmongkolkul}
\author{F.~C.~Porter}
\author{A.~Y.~Rakitin}
\affiliation{California Institute of Technology, Pasadena, California 91125, USA }
\author{R.~Andreassen}
\author{M.~S.~Dubrovin}
\author{G.~Mancinelli}
\author{B.~T.~Meadows}
\author{M.~D.~Sokoloff}
\affiliation{University of Cincinnati, Cincinnati, Ohio 45221, USA }
\author{P.~C.~Bloom}
\author{W.~T.~Ford}
\author{A.~Gaz}
\author{M.~Nagel}
\author{U.~Nauenberg}
\author{J.~G.~Smith}
\author{S.~R.~Wagner}
\affiliation{University of Colorado, Boulder, Colorado 80309, USA }
\author{R.~Ayad}\altaffiliation{Now at Temple University, Philadelphia, Pennsylvania 19122, USA }
\author{W.~H.~Toki}
\affiliation{Colorado State University, Fort Collins, Colorado 80523, USA }
\author{H.~Jasper}
\author{T.~M.~Karbach}
\author{J.~Merkel}
\author{A.~Petzold}
\author{B.~Spaan}
\author{K.~Wacker}
\affiliation{Technische Universit\"at Dortmund, Fakult\"at Physik, D-44221 Dortmund, Germany }
\author{M.~J.~Kobel}
\author{K.~R.~Schubert}
\author{R.~Schwierz}
\affiliation{Technische Universit\"at Dresden, Institut f\"ur Kern- und Teilchenphysik, D-01062 Dresden, Germany }
\author{D.~Bernard}
\author{M.~Verderi}
\affiliation{Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, F-91128 Palaiseau, France }
\author{P.~J.~Clark}
\author{S.~Playfer}
\author{J.~E.~Watson}
\affiliation{University of Edinburgh, Edinburgh EH9 3JZ, United Kingdom }
\author{M.~Andreotti$^{ab}$ }
\author{D.~Bettoni$^{a}$ }
\author{C.~Bozzi$^{a}$ }
\author{R.~Calabrese$^{ab}$ }
\author{A.~Cecchi$^{ab}$ }
\author{G.~Cibinetto$^{ab}$ }
\author{E.~Fioravanti$^{ab}$}
\author{P.~Franchini$^{ab}$ }
\author{E.~Luppi$^{ab}$ }
\author{M.~Munerato$^{ab}$}
\author{M.~Negrini$^{ab}$ }
\author{A.~Petrella$^{ab}$ }
\author{L.~Piemontese$^{a}$ }
\affiliation{INFN Sezione di Ferrara$^{a}$; Dipartimento di Fisica, Universit\`a di Ferrara$^{b}$, I-44100 Ferrara, Italy }
\author{R.~Baldini-Ferroli}
\author{A.~Calcaterra}
\author{R.~de~Sangro}
\author{G.~Finocchiaro}
\author{M.~Nicolaci}
\author{S.~Pacetti}
\author{P.~Patteri}
\author{I.~M.~Peruzzi}\altaffiliation{Also with Universit\`a di Perugia, Dipartimento di Fisica, Perugia, Italy }
\author{M.~Piccolo}
\author{M.~Rama}
\author{A.~Zallo}
\affiliation{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy }
\author{R.~Contri$^{ab}$ }
\author{E.~Guido$^{ab}$}
\author{M.~Lo~Vetere$^{ab}$ }
\author{M.~R.~Monge$^{ab}$ }
\author{S.~Passaggio$^{a}$ }
\author{C.~Patrignani$^{ab}$ }
\author{E.~Robutti$^{a}$ }
\author{S.~Tosi$^{ab}$ }
\affiliation{INFN Sezione di Genova$^{a}$; Dipartimento di Fisica, Universit\`a di Genova$^{b}$, I-16146 Genova, Italy  }
\author{B.~Bhuyan}
\author{V.~Prasad}
\affiliation{Indian Institute of Technology Guwahati, Guwahati, Assam, 781 039, India }
\author{C.~L.~Lee}
\author{M.~Morii}
\affiliation{Harvard University, Cambridge, Massachusetts 02138, USA }
\author{A.~Adametz}
\author{J.~Marks}
\author{U.~Uwer}
\affiliation{Universit\"at Heidelberg, Physikalisches Institut, Philosophenweg 12, D-69120 Heidelberg, Germany }
\author{F.~U.~Bernlochner}
\author{M.~Ebert}
\author{H.~M.~Lacker}
\author{T.~Lueck}
\author{A.~Volk}
\affiliation{Humboldt-Universit\"at zu Berlin, Institut f\"ur Physik, Newtonstr. 15, D-12489 Berlin, Germany }
\author{P.~D.~Dauncey}
\author{M.~Tibbetts}
\affiliation{Imperial College London, London, SW7 2AZ, United Kingdom }
\author{P.~K.~Behera}
\author{U.~Mallik}
\affiliation{University of Iowa, Iowa City, Iowa 52242, USA }
\author{C.~Chen}
\author{J.~Cochran}
\author{H.~B.~Crawley}
\author{L.~Dong}
\author{W.~T.~Meyer}
\author{S.~Prell}
\author{E.~I.~Rosenberg}
\author{A.~E.~Rubin}
\affiliation{Iowa State University, Ames, Iowa 50011-3160, USA }
\author{Y.~Y.~Gao}
\author{A.~V.~Gritsan}
\author{Z.~J.~Guo}
\affiliation{Johns Hopkins University, Baltimore, Maryland 21218, USA }
\author{N.~Arnaud}
\author{M.~Davier}
\author{D.~Derkach}
\author{J.~Firmino da Costa}
\author{G.~Grosdidier}
\author{F.~Le~Diberder}
\author{A.~M.~Lutz}
\author{B.~Malaescu}
\author{A.~Perez}
\author{P.~Roudeau}
\author{M.~H.~Schune}
\author{J.~Serrano}
\author{V.~Sordini}\altaffiliation{Also with  Universit\`a di Roma La Sapienza, I-00185 Roma, Italy }
\author{A.~Stocchi}
\author{L.~Wang}
\author{G.~Wormser}
\affiliation{Laboratoire de l'Acc\'el\'erateur Lin\'eaire, IN2P3/CNRS et Universit\'e Paris-Sud 11, Centre Scientifique d'Orsay, B.~P. 34, F-91898 Orsay Cedex, France }
\author{D.~J.~Lange}
\author{D.~M.~Wright}
\affiliation{Lawrence Livermore National Laboratory, Livermore, California 94550, USA }
\author{I.~Bingham}
\author{C.~A.~Chavez}
\author{J.~P.~Coleman}
\author{J.~R.~Fry}
\author{E.~Gabathuler}
\author{R.~Gamet}
\author{D.~E.~Hutchcroft}
\author{D.~J.~Payne}
\author{C.~Touramanis}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom }
\author{A.~J.~Bevan}
\author{F.~Di~Lodovico}
\author{R.~Sacco}
\author{M.~Sigamani}
\affiliation{Queen Mary, University of London, London, E1 4NS, United Kingdom }
\author{G.~Cowan}
\author{S.~Paramesvaran}
\author{A.~C.~Wren}
\affiliation{University of London, Royal Holloway and Bedford New College, Egham, Surrey TW20 0EX, United Kingdom }
\author{D.~N.~Brown}
\author{C.~L.~Davis}
\affiliation{University of Louisville, Louisville, Kentucky 40292, USA }
\author{A.~G.~Denig}
\author{M.~Fritsch}
\author{W.~Gradl}
\author{A.~Hafner}
\affiliation{Johannes Gutenberg-Universit\"at Mainz, Institut f\"ur Kernphysik, D-55099 Mainz, Germany }
\author{K.~E.~Alwyn}
\author{D.~Bailey}
\author{R.~J.~Barlow}
\author{G.~Jackson}
\author{G.~D.~Lafferty}
\author{T.~J.~West}
\affiliation{University of Manchester, Manchester M13 9PL, United Kingdom }
\author{J.~Anderson}
\author{R.~Cenci}
\author{A.~Jawahery}
\author{D.~A.~Roberts}
\author{G.~Simi}
\author{J.~M.~Tuggle}
\affiliation{University of Maryland, College Park, Maryland 20742, USA }
\author{C.~Dallapiccola}
\author{E.~Salvati}
\affiliation{University of Massachusetts, Amherst, Massachusetts 01003, USA }
\author{R.~Cowan}
\author{D.~Dujmic}
\author{P.~H.~Fisher}
\author{G.~Sciolla}
\author{M.~Zhao}
\affiliation{Massachusetts Institute of Technology, Laboratory for Nuclear Science, Cambridge, Massachusetts 02139, USA }
\author{D.~Lindemann}
\author{P.~M.~Patel}
\author{S.~H.~Robertson}
\author{M.~Schram}
\affiliation{McGill University, Montr\'eal, Qu\'ebec, Canada H3A 2T8 }
\author{P.~Biassoni$^{ab}$ }
\author{A.~Lazzaro$^{ab}$ }
\author{V.~Lombardo$^{a}$ }
\author{F.~Palombo$^{ab}$ }
\author{S.~Stracka$^{ab}$}
\affiliation{INFN Sezione di Milano$^{a}$; Dipartimento di Fisica, Universit\`a di Milano$^{b}$, I-20133 Milano, Italy }
\author{L.~Cremaldi}
\author{R.~Godang}\altaffiliation{Now at University of South Alabama, Mobile, Alabama 36688, USA }
\author{R.~Kroeger}
\author{P.~Sonnek}
\author{D.~J.~Summers}
\affiliation{University of Mississippi, University, Mississippi 38677, USA }
\author{X.~Nguyen}
\author{M.~Simard}
\author{P.~Taras}
\affiliation{Universit\'e de Montr\'eal, Physique des Particules, Montr\'eal, Qu\'ebec, Canada H3C 3J7  }
\author{G.~De Nardo$^{ab}$ }
\author{D.~Monorchio$^{ab}$ }
\author{G.~Onorato$^{ab}$ }
\author{C.~Sciacca$^{ab}$ }
\affiliation{INFN Sezione di Napoli$^{a}$; Dipartimento di Scienze Fisiche, Universit\`a di Napoli Federico II$^{b}$, I-80126 Napoli, Italy }
\author{G.~Raven}
\author{H.~L.~Snoek}
\affiliation{NIKHEF, National Institute for Nuclear Physics and High Energy Physics, NL-1009 DB Amsterdam, The Netherlands }
\author{C.~P.~Jessop}
\author{K.~J.~Knoepfel}
\author{J.~M.~LoSecco}
\author{W.~F.~Wang}
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA }
\author{L.~A.~Corwin}
\author{K.~Honscheid}
\author{R.~Kass}
\author{J.~P.~Morris}
\affiliation{Ohio State University, Columbus, Ohio 43210, USA }
\author{N.~L.~Blount}
\author{J.~Brau}
\author{R.~Frey}
\author{O.~Igonkina}
\author{J.~A.~Kolb}
\author{R.~Rahmat}
\author{N.~B.~Sinev}
\author{D.~Strom}
\author{J.~Strube}
\author{E.~Torrence}
\affiliation{University of Oregon, Eugene, Oregon 97403, USA }
\author{G.~Castelli$^{ab}$ }
\author{E.~Feltresi$^{ab}$ }
\author{N.~Gagliardi$^{ab}$ }
\author{M.~Margoni$^{ab}$ }
\author{M.~Morandin$^{a}$ }
\author{M.~Posocco$^{a}$ }
\author{M.~Rotondo$^{a}$ }
\author{F.~Simonetto$^{ab}$ }
\author{R.~Stroili$^{ab}$ }
\affiliation{INFN Sezione di Padova$^{a}$; Dipartimento di Fisica, Universit\`a di Padova$^{b}$, I-35131 Padova, Italy }
\author{E.~Ben-Haim}
\author{G.~R.~Bonneaud}
\author{H.~Briand}
\author{G.~Calderini}
\author{J.~Chauveau}
\author{O.~Hamon}
\author{Ph.~Leruste}
\author{G.~Marchiori}
\author{J.~Ocariz}
\author{J.~Prendki}
\author{S.~Sitt}
\affiliation{Laboratoire de Physique Nucl\'eaire et de Hautes Energies, IN2P3/CNRS, Universit\'e Pierre et Marie Curie-Paris6, Universit\'e Denis Diderot-Paris7, F-75252 Paris, France }
\author{M.~Biasini$^{ab}$ }
\author{E.~Manoni$^{ab}$ }
\author{A.~Rossi$^{ab}$ }
\affiliation{INFN Sezione di Perugia$^{a}$; Dipartimento di Fisica, Universit\`a di Perugia$^{b}$, I-06100 Perugia, Italy }
\author{C.~Angelini$^{ab}$ }
\author{G.~Batignani$^{ab}$ }
\author{S.~Bettarini$^{ab}$ }
\author{M.~Carpinelli$^{ab}$ }\altaffiliation{Also with Universit\`a di Sassari, Sassari, Italy}
\author{G.~Casarosa$^{ab}$ }
\author{A.~Cervelli$^{ab}$ }
\author{F.~Forti$^{ab}$ }
\author{M.~A.~Giorgi$^{ab}$ }
\author{A.~Lusiani$^{ac}$ }
\author{N.~Neri$^{ab}$ }
\author{E.~Paoloni$^{ab}$ }
\author{G.~Rizzo$^{ab}$ }
\author{J.~J.~Walsh$^{a}$ }
\affiliation{INFN Sezione di Pisa$^{a}$; Dipartimento di Fisica, Universit\`a di Pisa$^{b}$; Scuola Normale Superiore di Pisa$^{c}$, I-56127 Pisa, Italy }
\author{D.~Lopes~Pegna}
\author{C.~Lu}
\author{J.~Olsen}
\author{A.~J.~S.~Smith}
\author{A.~V.~Telnov}
\affiliation{Princeton University, Princeton, New Jersey 08544, USA }
\author{F.~Anulli$^{a}$ }
\author{E.~Baracchini$^{ab}$ }
\author{G.~Cavoto$^{a}$ }
\author{R.~Faccini$^{ab}$ }
\author{F.~Ferrarotto$^{a}$ }
\author{F.~Ferroni$^{ab}$ }
\author{M.~Gaspero$^{ab}$ }
\author{L.~Li~Gioi$^{a}$ }
\author{M.~A.~Mazzoni$^{a}$ }
\author{G.~Piredda$^{a}$ }
\author{F.~Renga$^{ab}$ }
\affiliation{INFN Sezione di Roma$^{a}$; Dipartimento di Fisica, Universit\`a di Roma La Sapienza$^{b}$, I-00185 Roma, Italy }
\author{T.~Hartmann}
\author{T.~Leddig}
\author{H.~Schr\"oder}
\author{R.~Waldi}
\affiliation{Universit\"at Rostock, D-18051 Rostock, Germany }
\author{T.~Adye}
\author{B.~Franek}
\author{E.~O.~Olaiya}
\author{F.~F.~Wilson}
\affiliation{Rutherford Appleton Laboratory, Chilton, Didcot, Oxon, OX11 0QX, United Kingdom }
\author{S.~Emery}
\author{G.~Hamel~de~Monchenault}
\author{G.~Vasseur}
\author{Ch.~Y\`{e}che}
\author{M.~Zito}
\affiliation{CEA, Irfu, SPP, Centre de Saclay, F-91191 Gif-sur-Yvette, France }
\author{M.~T.~Allen}
\author{D.~Aston}
\author{D.~J.~Bard}
\author{R.~Bartoldus}
\author{J.~F.~Benitez}
\author{C.~Cartaro}
\author{M.~R.~Convery}
\author{J.~Dorfan}
\author{G.~P.~Dubois-Felsmann}
\author{W.~Dunwoodie}
\author{R.~C.~Field}
\author{M.~Franco Sevilla}
\author{B.~G.~Fulsom}
\author{A.~M.~Gabareen}
\author{M.~T.~Graham}
\author{P.~Grenier}
\author{C.~Hast}
\author{W.~R.~Innes}
\author{M.~H.~Kelsey}
\author{H.~Kim}
\author{P.~Kim}
\author{M.~L.~Kocian}
\author{D.~W.~G.~S.~Leith}
\author{S.~Li}
\author{B.~Lindquist}
\author{S.~Luitz}
\author{V.~Luth}
\author{H.~L.~Lynch}
\author{D.~B.~MacFarlane}
\author{H.~Marsiske}
\author{D.~R.~Muller}
\author{H.~Neal}
\author{S.~Nelson}
\author{C.~P.~O'Grady}
\author{I.~Ofte}
\author{M.~Perl}
\author{T.~Pulliam}
\author{B.~N.~Ratcliff}
\author{A.~Roodman}
\author{A.~A.~Salnikov}
\author{V.~Santoro}
\author{R.~H.~Schindler}
\author{J.~Schwiening}
\author{A.~Snyder}
\author{D.~Su}
\author{M.~K.~Sullivan}
\author{S.~Sun}
\author{K.~Suzuki}
\author{J.~M.~Thompson}
\author{J.~Va'vra}
\author{A.~P.~Wagner}
\author{M.~Weaver}
\author{C.~A.~West}
\author{W.~J.~Wisniewski}
\author{M.~Wittgen}
\author{D.~H.~Wright}
\author{H.~W.~Wulsin}
\author{A.~K.~Yarritu}
\author{C.~C.~Young}
\author{V.~Ziegler}
\affiliation{SLAC National Accelerator Laboratory, Stanford, California 94309 USA }
\author{X.~R.~Chen}
\author{W.~Park}
\author{M.~V.~Purohit}
\author{R.~M.~White}
\author{J.~R.~Wilson}
\affiliation{University of South Carolina, Columbia, South Carolina 29208, USA }
\author{S.~J.~Sekula}
\affiliation{Southern Methodist University, Dallas, Texas 75275, USA }
\author{M.~Bellis}
\author{P.~R.~Burchat}
\author{A.~J.~Edwards}
\author{T.~S.~Miyashita}
\affiliation{Stanford University, Stanford, California 94305-4060, USA }
\author{S.~Ahmed}
\author{M.~S.~Alam}
\author{J.~A.~Ernst}
\author{B.~Pan}
\author{M.~A.~Saeed}
\author{S.~B.~Zain}
\affiliation{State University of New York, Albany, New York 12222, USA }
\author{N.~Guttman}
\author{A.~Soffer}
\affiliation{Tel Aviv University, School of Physics and Astronomy, Tel Aviv, 69978, Israel }
\author{P.~Lund}
\author{S.~M.~Spanier}
\affiliation{University of Tennessee, Knoxville, Tennessee 37996, USA }
\author{R.~Eckmann}
\author{J.~L.~Ritchie}
\author{A.~M.~Ruland}
\author{C.~J.~Schilling}
\author{R.~F.~Schwitters}
\author{B.~C.~Wray}
\affiliation{University of Texas at Austin, Austin, Texas 78712, USA }
\author{J.~M.~Izen}
\author{X.~C.~Lou}
\affiliation{University of Texas at Dallas, Richardson, Texas 75083, USA }
\author{F.~Bianchi$^{ab}$ }
\author{D.~Gamba$^{ab}$ }
\author{M.~Pelliccioni$^{ab}$ }
\affiliation{INFN Sezione di Torino$^{a}$; Dipartimento di Fisica Sperimentale, Universit\`a di Torino$^{b}$, I-10125 Torino, Italy }
\author{M.~Bomben$^{ab}$ }
\author{L.~Lanceri$^{ab}$ }
\author{L.~Vitale$^{ab}$ }
\affiliation{INFN Sezione di Trieste$^{a}$; Dipartimento di Fisica, Universit\`a di Trieste$^{b}$, I-34127 Trieste, Italy }
\author{N.~Lopez-March}
\author{F.~Martinez-Vidal}
\author{D.~A.~Milanes}
\author{A.~Oyanguren}
\affiliation{IFIC, Universitat de Valencia-CSIC, E-46071 Valencia, Spain }
\author{J.~Albert}
\author{Sw.~Banerjee}
\author{H.~H.~F.~Choi}
\author{K.~Hamano}
\author{G.~J.~King}
\author{R.~Kowalewski}
\author{M.~J.~Lewczuk}
\author{I.~M.~Nugent}
\author{J.~M.~Roney}
\author{R.~J.~Sobie}
\affiliation{University of Victoria, Victoria, British Columbia, Canada V8W 3P6 }
\author{T.~J.~Gershon}
\author{P.~F.~Harrison}
\author{T.~E.~Latham}
\author{E.~M.~T.~Puccio}
\affiliation{Department of Physics, University of Warwick, Coventry CV4 7AL, United Kingdom }
\author{H.~R.~Band}
\author{S.~Dasu}
\author{K.~T.~Flood}
\author{Y.~Pan}
\author{R.~Prepost}
\author{C.~O.~Vuosalo}
\author{S.~L.~Wu}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA }
\collaboration{The \babar\ Collaboration}
\noaffiliation


==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}




% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}
% add commands for NIM articles from earlier periods
% for NIM articles from 1981-1983
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\bf #1}}
% for NIM articles prior to 1981
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}


==> biblio.tex <==
\begin{thebibliography}{99}

%\cite{Aliev:2007gr}
\bibitem{Aliev:2007gr}
  T.~M.~Aliev, A.~S.~Cornell and N.~Gaur,
  %``B \to K(K^*) missing energy in Unparticle physics,''
  JHEP {\bf 0707}, 072 (2007).
%  [arXiv:0705.4542 [hep-ph]].
  %%CITATION = JHEPA,0707,072;%%

%\cite{Yamada:2007me}
\bibitem{Yamada:2007me}
  Y.~Yamada,
  %``$b \to s \nu \bar{\nu}$ decay in the MSSM: Implication of $b \to s \gamma$
  %at large tan $\beta$,''
  Phys.\ Rev.\  D {\bf 77}, 014025 (2008).
%  [arXiv:0709.1022 [hep-ph]].
  %%CITATION = PHRVA,D77,014025;%%

%\cite{Colangelo:2006vm}
\bibitem{Colangelo:2006vm}
  P.~Colangelo, F.~De Fazio, R.~Ferrandes and T.~N.~Pham,
  %``Exclusive B --> K(*) l+ l-, B --> K(*) nu anti-nu and B --> K* gamma
  %transitions in a scenario with a single universal extra dimension,''
  Phys.\ Rev.\  D {\bf 73}, 115006 (2006).
%  [arXiv:hep-ph/0604029].
  %%CITATION = PHRVA,D73,115006;%%

%\cite{Bird:2004ts}
\bibitem{Bird:2004ts}
  C.~Bird, P.~Jackson, R.~V.~Kowalewski and M.~Pospelov,
  %``Search for dark matter in b --> s transitions with missing energy,''
  Phys.\ Rev.\ Lett.\  {\bf 93}, 201803 (2004).
%  [arXiv:hep-ph/0401195].
  %%CITATION = PRLTA,93,201803;%%

%\cite{McKeen:2009rm}
\bibitem{McKeen:2009rm}
  D.~McKeen,
  %``WIMPless Dark Matter and Meson Decays with Missing Energy,''
  Phys.\ Rev.\  D {\bf 79}, 114001 (2009).
%  [arXiv:0903.4982 [hep-ph]].
  %%CITATION = PHRVA,D79,114001;%%

%\cite{Altmannshofer:2009ma}
\bibitem{Altmannshofer:2009ma}
  W.~Altmannshofer, A.~J.~Buras, D.~M.~Straub and M.~Wick,
  %``New strategies for New Physics search in $B \to K^{*} \nu \bar{\nu}$, $B
  %\to K \nu \bar{\nu}$ and $B \to X_{s} \nu \bar{\nu}$ decays,''
  JHEP {\bf 0904}, 022 (2009).
%  [arXiv:0902.0160 [hep-ph]].
  %%CITATION = JHEPA,0904,022;%%

%\cite{Buchalla:2000sk}
\bibitem{Buchalla:2000sk}
  G.~Buchalla, G.~Hiller and G.~Isidori,
  %``Phenomenology of nonstandard $Z$ couplings in exclusive semileptonic $b \to
  %s$ transitions,''
  Phys.\ Rev.\  D {\bf 63}, 014015 (2000).
%  [arXiv:hep-ph/0006136].
  %%CITATION = PHRVA,D63,014015;%%

%\cite{belle:2007zk}
\bibitem{belle:2007zk}
  K.~F.~Chen {\it et al.}  [BELLE Collaboration],
  %``Search for B -> h(*) nu nubar Decays at Belle,''
  Phys.\ Rev.\ Lett.\  {\bf 99}, 221802 (2007).
%  [arXiv:0707.0138 [hep-ex]].
  %%CITATION = PRLTA,99,221802;%%

%\cite{Aubert:2004ws}
\bibitem{Aubert:2004ws}
  B.~Aubert {\it et al.}  [\babar\ Collaboration],
  %``A search for the decay $B^+ \to K^+ \nu \bar{\nu}$,''
  Phys.\ Rev.\ Lett.\  {\bf 94}, 101801 (2005).
%  [arXiv:hep-ex/0411061].
  %%CITATION = PRLTA,94,101801;%%

%\cite{asterisk}
\bibitem{asterisk}
All kinematic quantities in this paper are defined in the lab frame unless 
marked with an asterisk, in which case they are in the CMS.


%\cite{Aubert:2001tu}
\bibitem{Aubert:2001tu}
  B.~Aubert {\it et al.} [\babar\ Collaboration],
  %``The BaBar detector,''
  Nucl.\ Instrum.\ Meth.\  A {\bf 479}, 1 (2002).
%  [arXiv:hep-ex/0105044].
  %%CITATION = NUIMA,A479,1;%%

%\cite{Aubert:2009rk}
\bibitem{Aubert:2009rk}
  B.~Aubert {\it et al.}  [\babar\ Collaboration],
  %``Search for the Rare Leptonic Decays \boldmath{\Blnu} ($\ell=e,\mu$),''
  Phys.\ Rev.\  D {\bf 79}, 091101 (2009).
%  [arXiv:0903.1220 [hep-ex]].
  %%CITATION = PHRVA,D79,091101;%%

%\cite{Aubert:2007bx}
\bibitem{Aubert:2007bx}
  B.~Aubert {\it et al.}  [\babar\ Collaboration],
  %``A Search for $B^{+} \to \tau^{+} \nu$,''
  Phys.\ Rev.\  D {\bf 76}, 052002 (2007).
%  [arXiv:0705.1820 [hep-ex]].
  %%CITATION = PHRVA,D76,052002;%%
  
\bibitem{Aubert:2004}
  B.~Aubert {\it et al.}  [\babar\ Collaboration],
  Phys.\ Rev.\ Lett.\ {\bf 94}, 101801 (2005). 
   
\bibitem{pdg:2008}
        C. Amsler {\it et al.} [Particle Data Group],
        Physics Letters B, \textbf{667}, 1 (2008).
        
%\cite{Breiman}
\bibitem{Breiman}
  L.~Breiman,
  %``Bagging predictors$,''
  Mach. Learn. {\bf 24}, 2 (1996).

%\cite{Narsky:2005hn}
\bibitem{Narsky:2005hn}
  I.~Narsky,
  %``Optimization of signal significance by bagging decision trees,''
  arXiv:physics/0507157 (2005).
  %%CITATION = PHYSICS/0507157;%%

%\cite{Agostinelli:2002hh}
\bibitem{Agostinelli:2002hh}
  S.~Agostinelli {\it et al.}  [GEANT4 Collaboration],
  %``GEANT4: A simulation toolkit,''
  Nucl.\ Instrum.\ Meth.\  A {\bf 506}, 250 (2003).
  %%CITATION = NUIMA,A506,250;%%

%\cite{Bootstrap}
\bibitem{Bootstrap}
  B.~Efron and R.~Tibshirani,
  \emph{An Introduction to the Bootstrap},
  Chapman \& Hall (1993).

%\cite{Barlow}
\bibitem{Barlow}
  R.~Barlow,
  \emph{Application of the Bootstrap Resampling Technique to Particle Physics Experiments},
  Preprint MAN-HEP-99-4, (2000), www.hep.manchester.ac.uk/preprints/archive.html.

\bibitem{Barlow2}
  R.~Barlow,
  Computer Physics Communications {\bf 149}, 97 (2002).
\end{thebibliography}


==> symbols.tex <==
% Additional symbols used in this document.
\def \eff{\hbox{eff}}
\newcommand{\gevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\def\BtoJpsiK {\ensuremath{B\to J/\psi K^{(*)}}\xspace}
\def\D {\ensuremath{D}\xspace}
\def\K {\ensuremath{K}\xspace}
\def\mKpi {\ensuremath{m_{K\pi}}\xspace}
\def\KTight {\textit{Tight}\xspace}
\def\KVeryTight {\textit{VeryTight}\xspace}
\def\Kmaybestar {\ensuremath{K^{(*)}\xspace}}
\def\Dmaybestar {\ensuremath{D^{(*)}\xspace}}
\def\costhb {\ensuremath{\cos\theta_B}\xspace}
\def\cosththr {\ensuremath{\cos\theta_{\rm thrust}}\xspace}
\def\cosththrROE {\ensuremath{\cos\theta_{\rm thrust_{\rm ROE}}}\xspace}
\def\costhst {\ensuremath{\cos\theta^*}\xspace}
%\def\emu {\ensuremath{e\mu}\xspace}
\def\fskee {\ensuremath{K^\pm\epem}\xspace}
\def\fskmm {\ensuremath{K^\pm\mumu}\xspace}
\def\fskll {\ensuremath{K^\pm\ellell}\xspace}
\def\fsksee {\ensuremath{K^0_{\scriptscriptstyle S}\epem}\xspace}
\def\fsksmm {\ensuremath{K^0_{\scriptscriptstyle S}\mumu}\xspace}
\def\fskstkee {\ensuremath{K^{*0}\epem}\xspace}
\def\fskstkmm {\ensuremath{K^{*0}\mumu}\xspace}
\def\fskstkll {\ensuremath{K^{*0}\ellell}\xspace}
\def\fskstksee {\ensuremath{K^{*\pm}\epem}\xspace}
\def\fskstksmm {\ensuremath{K^{*\pm}\mumu}\xspace}
\def\fskstksll {\ensuremath{K^{*\pm}\ellell}\xspace}
\def\fskstll {\ensuremath{K^{*}\ellell}\xspace}
\def\jpsimodes {\B\to\jpsi \Kmaybestar \xspace}
\def\jpsik {\ensuremath{\B\to\jpsi K \xspace}}
\def\jpsikstk {\ensuremath{\B\to\jpsi K^{*0}\xspace}}
\def\kmaybell {\B\to\Kmaybestar\ellell\xspace}
\def\modekmaybell {\B\to\Kmaybestar\ellell\xspace}
\def\kmaybemm {\B\to\Kmaybestar\mumu\xspace}
\def\mklep {\ensuremath{m_{K\ell}}\xspace}
\def\mkpi {\ensuremath{m_{\kaon\pi}}\xspace}
\def\mll {\ensuremath{m_{\ell\ell}}\xspace}
\def\ctl {\ensuremath{\cos\theta_{\ell}}\xspace}
\def\stl {\ensuremath{\sin\theta_{\ell}}\xspace}
\def\ctlsq {\ensuremath{\cos^2\theta_{\ell}}\xspace}
\def\stlsq {\ensuremath{\sin^2\theta_{\ell}}\xspace}
\def\ctk {\ensuremath{\cos\theta_{K}}\xspace}
\def\stk {\ensuremath{\sin\theta_{K}}\xspace}
\def\ctksq {\ensuremath{\cos^2\theta_{K}}\xspace}
\def\stksq {\ensuremath{\sin^2\theta_{K}}\xspace}
\def\ak {\ensuremath{\alpha_{K^*}}\xspace}
\def\modekJpsill {\ensuremath{\Bp \to K^+ J/\psi(\to \ellell)}\xspace}
\def\modekshJpsill {\ensuremath{\Bz \to \KS J/\psi(\to \ellell)}\xspace}
\def\modekpsitwosll {\ensuremath{\B^+\to K^+ \psitwos(\to \ellell)}\xspace}
\def\modekshpsitwosll {\ensuremath{\B^+\to \KS \psitwos(\to \ellell)}\xspace}
\def\modekavgll {\ensuremath{B\to K\ellell}\xspace}
\def\modekavgee {\ensuremath{B\to K\epem}\xspace}
\def\modekavgmm {\ensuremath{B\to K\mumu}\xspace}
\def\modekavgnn {\ensuremath{B \to K\nunub}\xspace}
\def\modekstnn {\ensuremath{B_{d}\to K^{*}\nunub}\xspace}
\def\modekplnn {\ensuremath{B^{+}\to K^{+}\nunub}\xspace}
\def\modekstavgnn {\ensuremath{B \to K^{*}\nunub}\xspace}
\def\modekzeronn {\ensuremath{B^{0}\to K^{0}_{S}\nunub}\xspace}
\def\modekavgem {\ensuremath{B\to K\emu}\xspace}
\def\modekstem {\ensuremath{B\to K^{*}\emu}\xspace}
\def\modekee {\ensuremath{B^+\rightarrow K^+\epem}\xspace}
\def\modekem {\ensuremath{B^+\rightarrow K^+\emu}\xspace}
\def\modekxem {\ensuremath{B^+\rightarrow K^+ e^\pm \mu^\mp}\xspace}
\def\modekxme {\ensuremath{B^+\rightarrow K^+ \mu^\pm e^\mp}\xspace}
\def\modekll {\ensuremath{B^+\rightarrow K^+\ellell}\xspace}
\def\modekmm {\ensuremath{B^+\rightarrow K^+\mumu}\xspace}
\def\modeksJpsill {\ensuremath{B^0\rightarrow K^0 J/\psi(\rightarrow\ellell)}\xspace}
\def\modeksee {\ensuremath{B^0\rightarrow K^0_{\scriptscriptstyle S}\epem}\xspace}
\def\modeksem {\ensuremath{B^0\rightarrow K^0_{\scriptscriptstyle S}\emu}\xspace}
\def\modekzem {\ensuremath{B^0\rightarrow K^0\emu}\xspace}
\def\modeksll {\ensuremath{B^0\rightarrow K^0_{\scriptscriptstyle S}\ellell}\xspace}
\def\modeksmm {\ensuremath{B^0\rightarrow K^0_{\scriptscriptstyle S}\mumu}\xspace}
\def\modekstee {\ensuremath{B\rightarrow K^{*}\epem}\xspace}
\def\modekstll {\ensuremath{B\rightarrow K^{*}\ellell}\xspace}
\def\modekstmm {\ensuremath{B\rightarrow K^{*}\mumu}\xspace}
\def\modekstkJpsill {\ensuremath{B^0\rightarrow K^{*0} J/\psi(\rightarrow\ellell)}\xspace}
\def\modekstkpsitwosll {\ensuremath{B^0\rightarrow K^{*0} \psitwos(\rightarrow\ellell)}\xspace}
\def\modekstkee {\ensuremath{B^0\rightarrow K^{*0}\epem}\xspace}
\def\modekstkem {\ensuremath{B^0\rightarrow K^{*0}\emu}\xspace}
\def\modekstkxem {\ensuremath{B^0\rightarrow K^{*0} e^\pm \mu^\mp}\xspace}
\def\modekstkxme {\ensuremath{B^0\rightarrow K^{*0} \mu^\pm e^\mp}\xspace}
\def\modekstkll {\ensuremath{B^0\rightarrow K^{*0}\ellell}\xspace}
\def\modekstkmm {\ensuremath{B^0\rightarrow K^{*0}\mumu}\xspace}
\def\modekstksJpsill {\ensuremath{B^+\rightarrow K^{*+}J/\psi(\rightarrow\ellell)}\xspace}
\def\modekstkspsitwosll {\ensuremath{B^+\rightarrow K^{*+}\psitwos(\rightarrow\ellell)}\xspace}
\def\modekstksee {\ensuremath{B^+\rightarrow K^{*+}\epem}\xspace}
\def\modekstksem {\ensuremath{B^+\rightarrow K^{*+}\emu}\xspace}
\def\modekstksxem {\ensuremath{B^+\rightarrow K^{*+}e^\pm \mu^\mp}\xspace}
\def\modekstksxme {\ensuremath{B^+\rightarrow K^{*+}\mu^\pm e^\mp}\xspace}
\def\modekstksll {\ensuremath{B^+\rightarrow K^{*+}\ellell}\xspace}
\def\modekstksmm {\ensuremath{B^+\rightarrow K^{*+}\mumu}\xspace}
\def\modekzee {\ensuremath{B^0\rightarrow K^0\epem}\xspace}
\def\modekzll {\ensuremath{B^0\rightarrow K^0\ellell}\xspace}
\def\modekzmm {\ensuremath{B^0\rightarrow K^0\mumu}\xspace}
\def\modekstzee {\ensuremath{B^0\rightarrow K^{*0}\epem}\xspace}
\def\modekstzll {\ensuremath{B^0\rightarrow K^{*0}\ellell}\xspace}
\def\modekstzmm {\ensuremath{B^0\rightarrow K^{*0}\mumu}\xspace}
\def\mupm {\ensuremath{\mu^\pm}\xspace}
\def\runone {Run~1\xspace}
\def\runtwo {Run~2\xspace}
\def\runthree {Run~3\xspace}
\def\runfour {Run~4\xspace}
\def\runfive {Run~5\xspace}
\def\uds {\ensuremath{uds}\xspace}
\def\vs {\textit{vs.}\xspace}
\def\mesROE {\mbox{$m_{\rm ES}^{ROE}$}\xspace}
\def\DeltaEROE {\mbox{$\Delta E^{ROE}$}\xspace}
\def\cosththrroe {\mbox{$\cos\theta_{thr}^{ROE}$}\xspace}
\def\afb {\mbox{${\cal A}_{FB}$}\xspace}
\def\fl {\mbox{$F_L$}\xspace}
\def\invab {\ensuremath{\mbox{\,ab}^{-1}}\xspace}
\def\modekpizmm {\ensuremath{B^+\rightarrow \Kp \piz \mumu}\xspace}
\def\modekspipmm {\ensuremath{B^+\rightarrow \KS \pip \mumu}\xspace}
\def\modekppimmm {\ensuremath{B^0\rightarrow \Kp \pim \mumu}\xspace}
\def\modekpizee {\ensuremath{B^+\rightarrow \Kp \piz \epem}\xspace}
\def\modekspipee {\ensuremath{B^+\rightarrow \KS \pip \epem}\xspace}
\def\modekppimee {\ensuremath{B^0\rightarrow \Kp \pim \epem}\xspace}
\def\modeone {\ensuremath{B^0\rightarrow \KS \mumu}\xspace}
\def\modetwo {\ensuremath{B^+\rightarrow K^+\mumu}\xspace}
\def\modethree {\ensuremath{B^0\rightarrow \KS \epem}\xspace}
\def\modefour {\ensuremath{B^+\rightarrow K^+\epem}\xspace}
\def\modefive {\ensuremath{B^0\rightarrow \KS \piz \mumu}\xspace}
\def\modesix {\ensuremath{B^+\rightarrow \Kp \piz \mumu}\xspace}
\def\modeseven {\ensuremath{B^+\rightarrow \KS \pip \mumu}\xspace}
\def\modeeight {\ensuremath{B^0\rightarrow \Kp \pim \mumu}\xspace}
\def\modenine {\ensuremath{B^0\rightarrow \KS \piz \epem}\xspace}
\def\modeten {\ensuremath{B^+\rightarrow \Kp \piz \epem}\xspace}
\def\modeeleven {\ensuremath{B^+\rightarrow \KS \pip \epem}\xspace}
\def\modetwelve {\ensuremath{B^0\rightarrow \Kp \pim \epem}\xspace}
\def\lfvone {\ensuremath{B^0\rightarrow \KS \mue}\xspace}
\def\lfvtwo {\ensuremath{B^+\rightarrow K^+\mue}\xspace}
\def\lfvthree {\ensuremath{B^0\rightarrow \KS \emu}\xspace}
\def\lfvfour {\ensuremath{B^+\rightarrow K^+\emu}\xspace}
\def\lfvfive {\ensuremath{B^+\rightarrow \KS \piz \mue}\xspace}
\def\lfvsix {\ensuremath{B^+\rightarrow \Kp \piz \mue}\xspace}
\def\lfvseven {\ensuremath{B^+\rightarrow \KS \pip \mue}\xspace}
\def\lfveight {\ensuremath{B^0\rightarrow \Kp \pim \mue}\xspace}
\def\lfvnine {\ensuremath{B^0\rightarrow \KS \piz \emu}\xspace}
\def\lfvten {\ensuremath{B^+\rightarrow \Kp \piz \emu}\xspace}
\def\lfveleven {\ensuremath{B^+\rightarrow \KS \pip \emu}\xspace}
\def\lfvtwelve {\ensuremath{B^0\rightarrow \Kp \pim \emu}\xspace}
\def\BBbar {\ensuremath{B\Bbar}}
\def\modekzeroallnn {\ensuremath{B^{0}\to K^{0}\nunub}\xspace}
\def\Bsig {\ensuremath{B_{\rm roe}}}
\def\Btag {\ensuremath{B_{\rm rec}}}
\def\Eex {\ensuremath{E_{\rm extra}}}
\def\mnn {\ensuremath{q^{2}}}
